Differentially Private Synthetic Data: Applied Evaluations and Enhancements

Machine learning practitioners frequently seek to leverage the most informative available data, without violating the data owner's privacy, when building predictive models. Differentially private data synthesis protects personal details from exposure, and allows for the training of differentially private machine learning models on privately generated datasets. But how can we effectively assess the efficacy of differentially private synthetic data? In this paper, we survey four differentially private generative adversarial networks for data synthesis. We evaluate each of them at scale on five standard tabular datasets, and in two applied industry scenarios. We benchmark with novel metrics from recent literature and other standard machine learning tools. Our results suggest some synthesizers are more applicable for different privacy budgets, and we further demonstrate complicating domain-based tradeoffs in selecting an approach. We offer experimental learning on applied machine learning scenarios with private internal data to researchers and practioners alike. In addition, we propose QUAIL, an ensemble-based modeling approach to generating synthetic data. We examine QUAIL's tradeoffs, and note circumstances in which it outperforms baseline differentially private supervised learning models under the same budget constraint.

==> email.tex <==
Hi Vijay and Soundar!

As you are all aware, Anuj, Eddie, Samira, April and I have been putting together an ICLR submission as part of the continued collaboration between MAIDAP, COSINE and AI Platform Responsible AI. The paper is provisionally titled “Evaluating and Enhancing the Applied Performance of DP Synthetic Data,” and details our work on evaluating 4 SOTA differentially private (DP) synthesizers, new metrics from recent literature, and QUAIL, a novel enhancement to DP synthesis for ML tasks in standard and applied settings.

We are asking each of you for feedback on the first draft of our submission, which is attached in PDF form (and linked here on Overleaf: https://www.overleaf.com/read/czmmrgxycvfm).

The abstract submission deadline is September 28th, with the full draft due on October 2nd. This should leave enough time for you to take a look at the draft over the course of next week. We will be setting up a short meeting next Thursday/Friday to discuss. We look forward to incorporating your feedback into the camera ready copy!

We are specifically looking for feedback in these areas:
- Does the paper present a particular narrative that you found compelling/impactful, that we should do more to highlight?
- Conversely, does anything presented distract from the content you found compelling/impactful?
- We have some reservations about the difficulty of hyperparameter tuning, which we are trying to improve on before submission. As it currently stands, do we adequately address the topic?
- Soundar: As an ICLR reviewer, are there changes we could make to improve our chances at being accepted at this specific venue?

Thank you both so much,

Anuj, Eddie, Samira, April and Lucas

Hi Sergey, __, __!

As you are all aware, Anuj, Eddie, Samira, April and I have been putting together an ICLR submission as part of the continued collaboration between MAIDAP, COSINE and AI Platform Responsible AI. The paper is provisionally titled “Evaluating and Enhancing the Applied Performance of DP Synthetic Data,” and details our work on evaluating 4 SOTA differentially private (DP) synthesizers, new metrics from recent literature, and QUAIL, a novel enhancement to DP synthesis for ML tasks in standard and applied settings.

We are asking each of you for feedback on the first draft of our submission, which is attached in PDF form (and linked here on Overleaf: https://www.overleaf.com/read/czmmrgxycvfm).

The abstract submission deadline is September 28th, with the full draft due on October 2nd. This should leave enough time for you to take a look at the draft over the course of next week. We will be setting up a short meeting next Thursday/Friday to discuss. We look forward to incorporating your feedback into the camera ready copy!

We are specifically looking for feedback in these overall areas:
- Does the paper present a particular narrative that you found compelling/impactful, that we should do more to highlight?
- Conversely, does anything presented distract from the content you found compelling/impactful?
- We have some reservations about the difficulty of hyperparameter tuning, which we are trying to improve on before submission. As it currently stands, do we adequately address the topic?
- As people more familiar with ICLR as a venue, are there changes we could make to improve our chances at being accepted at this specific venue?

With your DP expertise, we would also love feedback on our implementation details:
- We applied DP-SGD to CTGAN and wanted to know whether you can validate (formally or informally : ) ) that this implementation (DP-CTGAN) preserves differential privacy. In terms of implementation, we add noise and clip norm on discriminator. The CTGAN paper is here: https://arxiv.org/pdf/1907.00503.pdf. You can look at the section 4.3 (Conditional Generator and Training-by-Sampling) directly. Our implementation of DP-CTGAN is here: https://github.com/opendifferentialprivacy/whitenoise-system/blob/master/sdk/opendp/whitenoise/synthesizers/pytorch/nn/dpctgan.py.  

- We also applied the PATE framework to CTGAN and wanted to know whether our implementation of this PATE-CTGAN is differentially preserved. The architecture is very similar to PATE-GAN (https://openreview.net/forum?id=S1zk9iRqF7), except the procedure of training teacher discriminator.  For the procedure of training teacher discriminator, we initialized k conditional generator for each subset of data. The implementation of patectgan can be found here https://github.com/opendifferentialprivacy/whitenoise-system/blob/master/sdk/opendp/whitenoise/synthesizers/pytorch/nn/patectgan.py


Thank you all so much,

Anuj, Eddie, Samira, April and Lucas

Hi Joshua!

As you well aware, Anuj, Eddie, Samira, April and I have been putting together an ICLR submission as part of the continued collaboration between MAIDAP, COSINE and AI Platform Responsible AI. The paper is provisionally titled “Evaluating and Enhancing the Applied Performance of DP Synthetic Data,” and details our work on evaluating 4 SOTA differentially private (DP) synthesizers, new metrics from recent literature, and QUAIL, a novel enhancement to DP synthesis for ML tasks in standard and applied settings.

We are asking each of you for feedback on the first draft of our submission, which is attached in PDF form (and linked here on Overleaf: https://www.overleaf.com/read/czmmrgxycvfm).

The abstract submission deadline is September 28th, with the full draft due on October 2nd. This should leave enough time for you to take a look at the draft over the course of next week. We will be setting up a short meeting next Thursday/Friday to discuss. We look forward to incorporating your feedback into the camera ready copy!

We are specifically looking for feedback in these overall areas:
- Does the paper present a particular narrative that you found compelling/impactful, that we should do more to highlight?
- Conversely, does anything presented distract from the content you found compelling/impactful?
- We have some reservations about the difficulty of hyperparameter tuning, which we are trying to improve on before submission. As it currently stands, do we adequately address the topic?
- As people more familiar with ICLR as a venue, are there changes we could make to improve our chances at being accepted at this specific venue?

With your DP expertise, we would also love feedback on our implementation details:
- We applied DP-SGD to CTGAN and wanted to know whether you can validate (formally or informally : ) ) that this implementation (DP-CTGAN) preserves differential privacy. In terms of implementation, we add noise and clip norm on discriminator. The CTGAN paper is here: https://arxiv.org/pdf/1907.00503.pdf. You can look at the section 4.3 (Conditional Generator and Training-by-Sampling) directly. Our implementation of DP-CTGAN is here: https://github.com/opendifferentialprivacy/whitenoise-system/blob/master/sdk/opendp/whitenoise/synthesizers/pytorch/nn/dpctgan.py.  

- We also applied the PATE framework to CTGAN and wanted to know whether our implementation of this PATE-CTGAN is differentially preserved. The architecture is very similar to PATE-GAN (https://openreview.net/forum?id=S1zk9iRqF7), except the procedure of training teacher discriminator.  For the procedure of training teacher discriminator, we initialized k conditional generator for each subset of data. The implementation of patectgan can be found here https://github.com/opendifferentialprivacy/whitenoise-system/blob/master/sdk/opendp/whitenoise/synthesizers/pytorch/nn/patectgan.py


Thank you all so much,

Anuj, Eddie, Samira, April and Lucas
